Differentiable Particle Optimization for Fast Sequential Manipulation

Sequential robot manipulation tasks require finding collision-free trajectories that satisfy geometric constraints across multiple object interactions in potentially high-dimensional configuration spaces. Solving these problems in real-time and at large scales has remained out of reach due to computational requirements. Recently, GPU-based acceleration has shown promising results, but prior methods achieve limited performance due to CPU-GPU data transfer overhead and complex logic that prevents full hardware utilization. To this end, we present SPaSM (Sampling Particle optimization for Sequential Manipulation), a fully GPU-parallelized framework that compiles constraint evaluation, sampling, and gradient-based optimization into optimized CUDA kernels for end-to-end trajectory optimization without CPU coordination. The method consists of a two-stage particle optimization strategy: first solving placement constraints through massively parallel sampling, then lifting solutions to full trajectory optimization in joint space. Unlike hierarchical approaches, SPaSM jointly optimizes object placements and robot trajectories to handle scenarios where motion feasibility constrains placement options. Experimental evaluation on challenging benchmarks demonstrates solution times in the realm of $\textbf{milliseconds}$ with a 100% success rate; a $4000\times$ speedup compared to existing approaches. Code and examples are available at $\href{https://commalab.org/papers/spasm}{commalab.org/papers/spasm}$.

==> 5table.tex <==

\begin{table}
    \centering
    
    \begin{tabular}{lrrr}
        \toprule
        \textbf{Approach} & $N_b$ & \textbf{Coverage} & \textbf{Sol. Time (s)} \\
        % \midrule
        % \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM + TrajOpt}} 
        % & 512 & 100/100 & \textbf{3.74 ± 2.31 ms} \\
        % & 1024 & 100/100 & 3.76 ± 2.25 ms \\
        % & 2048 & 100/100 & 4.32 ± 1.88 ms \\
        % & 4096 & 100/100 & 6.39 ± 1.92 ms \\
        % & 8192 & 100/100 & 12.45 ± 2.14 ms \\
        % \midrule
        % \multirow{5}{*}{\parbox{1.35cm}{\scshape cuTAMP + CuRobo \\ (tuned)}} 
        % & 512 & 30/30 & 18.98 ± 6.80 s \\
        % & 1024 & 30/30 & 12.14 ± 2.92 s \\
        % & 2048 & 30/30 & \textbf{7.33 ± 0.93 s} \\
        % & 4096 & 30/30 & 9.01 ± 1.10 s \\
        % & 8192 & 30/30 & 11.88 ± 0.98 s \\
        \midrule
        \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSm w/o TrajOpt \\ (tuned)}} 
        & 512 & 30/30 & 18.98 ± 6.80 s \\
        & 1024 & 30/30 & 12.14 ± 2.92 s \\
        & 2048 & 30/30 & \textbf{7.33 ± 0.93 s} \\
        & 4096 & 30/30 & 9.01 ± 1.10 s \\
        & 8192 & 30/30 & 11.88 ± 0.98 s \\
        \midrule
        \multirow{5}{*}{\parbox{1.35cm}{\scshape cuTAMP only\\ (tuned)}} 
        & 512 & 30/30 & 18.98 ± 6.80 s \\
        & 1024 & 30/30 & 12.14 ± 2.92 s \\
        & 2048 & 30/30 & \textbf{7.33 ± 0.93 s} \\
        & 4096 & 30/30 & 9.01 ± 1.10 s \\
        & 8192 & 30/30 & 11.88 ± 0.98 s \\
        \bottomrule
    \end{tabular}

    \begin{tabular}{lrrr}
        \toprule
        \textbf{Approach} & $N_b$ & \textbf{Coverage} & \textbf{Sol. Time (s)} \\
        % \midrule
        % \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM + TrajOpt}} 
        % & 512 & 100/100 & \textbf{3.74 ± 2.31 ms} \\
        % & 1024 & 100/100 & 3.76 ± 2.25 ms \\
        % & 2048 & 100/100 & 4.32 ± 1.88 ms \\
        % & 4096 & 100/100 & 6.39 ± 1.92 ms \\
        % & 8192 & 100/100 & 12.45 ± 2.14 ms \\
        % \midrule
        % \multirow{5}{*}{\parbox{1.35cm}{\scshape cuTAMP + CuRobo \\ (tuned)}} 
        % & 512 & 30/30 & 18.98 ± 6.80 s \\
        % & 1024 & 30/30 & 12.14 ± 2.92 s \\
        % & 2048 & 30/30 & \textbf{7.33 ± 0.93 s} \\
        % & 4096 & 30/30 & 9.01 ± 1.10 s \\
        % & 8192 & 30/30 & 11.88 ± 0.98 s \\
        \midrule
        \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSm w/o TrajOpt \\ (tuned)}} 
        & 512 & 30/30 & 18.98 ± 6.80 s \\
        & 1024 & 30/30 & 12.14 ± 2.92 s \\
        & 2048 & 30/30 & \textbf{7.33 ± 0.93 s} \\
        & 4096 & 30/30 & 9.01 ± 1.10 s \\
        & 8192 & 30/30 & 11.88 ± 0.98 s \\
        \midrule
        \multirow{5}{*}{\parbox{1.35cm}{\scshape cuTAMP only\\ (tuned)}} 
        & 512 & 30/30 & 18.98 ± 6.80 s \\
        & 1024 & 30/30 & 12.14 ± 2.92 s \\
        & 2048 & 30/30 & \textbf{7.33 ± 0.93 s} \\
        & 4096 & 30/30 & 9.01 ± 1.10 s \\
        & 8192 & 30/30 & 11.88 ± 0.98 s \\
        \bottomrule
    \end{tabular}


    \caption{5 tetris time to first solution with fixed skeleton. Should we extend the batches for SPaSM? (cutamp only goes to 8192 since it takes really long and the original paper just goes to 4096 anyway}
    \label{tab:5table}
\end{table}

==> 8table.tex <==

\begin{figure}
    \centering

    \textcolor{blue}{note: add quadratic cost DNF here}

    \begin{tabular}{lrrr}
    \toprule
    \textbf{Approach} & $N_b$ & \textbf{Coverage} & \textbf{Sol. Time} \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM + TrajOpt}} 
    & 512 & 100/100 & 13.87 ± 7.31 ms \\
    & 1024 & 100/100 & \textbf{12.43 ± 4.96 ms} \\
    & 2048 & 100/100 & 15.84 ± 4.55 ms \\
    & 4096 & 100/100 & 34.73 ± 4.13 ms \\
    & 8192 & 100/100 & 84.71 ± 4.81 ms \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape cuTAMP + CuRobo \\ (Tuned)}} 
    & 512 & 4/5 & \textbf{65.48 ± 30.38 s} \\
    & 1024 & 25/30 & 133.69 ± 61.31 s \\
    & 2048 & 30/30 & 119.91 ± 49.12 s \\
    & 4096 & 30/30 & 74.58 ± 15.15 s \\
    & 8192 & 30/30 & 90.06 ± 19.74 s \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSm w/o TrajOpt  \\ (Tuned)}} 
    & 512 & 4/5 & \textbf{65.48 ± 30.38 s} \\
    & 1024 & 25/30 & 133.69 ± 61.31 s \\
    & 2048 & 30/30 & 119.91 ± 49.12 s \\
    & 4096 & 30/30 & 74.58 ± 15.15 s \\
    & 8192 & 30/30 & 90.06 ± 19.74 s \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape cuTAMP only \\ (Tuned)}} 
    & 512 & 4/5 & \textbf{65.48 ± 30.38 s} \\
    & 1024 & 25/30 & 133.69 ± 61.31 s \\
    & 2048 & 30/30 & 119.91 ± 49.12 s \\
    & 4096 & 30/30 & 74.58 ± 15.15 s \\
    & 8192 & 30/30 & 90.06 ± 19.74 s \\
    \bottomrule
    \end{tabular}

    \caption{8 tetris time to first solution with fixed skeleton. We ran cutamp trials for up to THIRTY THOUSAND steps each, and despite that some trials fail (coverage is what cutamp people call success in their paper). (They don't mention how many steps in the original so i think 30,000 is safe)}
    \label{fig:8table}
\end{figure}

==> towertable.tex <==


\begin{figure}
    \centering

    \textbf{Tower Stacking without Obstacles}
    \begin{tabular}{lrrr}
    \toprule
    \textbf{Approach} & $N_b$ & \textbf{Coverage} & \textbf{Sol. Time} \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM w/o TrajOpt }} 
    & 512 & 100/100 & 13.87 ± 7.31 ms \\
    & 1024 & 100/100 & \textbf{12.43 ± 4.96 ms} \\
    & 2048 & 100/100 & 15.84 ± 4.55 ms \\
    & 4096 & 100/100 & 34.73 ± 4.13 ms \\
    & 8192 & 100/100 & 84.71 ± 4.81 ms \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM + TrajOpt}} 
    & 512 & 4/5 & \textbf{65.48 ± 30.38 s} \\
    & 1024 & 25/30 & 133.69 ± 61.31 s \\
    & 2048 & 30/30 & 119.91 ± 49.12 s \\
    & 4096 & 30/30 & 74.58 ± 15.15 s \\
    & 8192 & 30/30 & 90.06 ± 19.74 s \\
    \bottomrule
    \end{tabular}

    \textbf{Tower Stacking with one Obstacles}
    \begin{tabular}{lrrr}
    \toprule
    \textbf{Approach} & $N_b$ & \textbf{Coverage} & \textbf{Sol. Time} \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM w/o TrajOpt }} 
    & 512 & 100/100 & 13.87 ± 7.31 ms \\
    & 1024 & 100/100 & \textbf{12.43 ± 4.96 ms} \\
    & 2048 & 100/100 & 15.84 ± 4.55 ms \\
    & 4096 & 100/100 & 34.73 ± 4.13 ms \\
    & 8192 & 100/100 & 84.71 ± 4.81 ms \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM + TrajOpt }} 
    & 512 & 4/5 & \textbf{65.48 ± 30.38 s} \\
    & 1024 & 25/30 & 133.69 ± 61.31 s \\
    & 2048 & 30/30 & 119.91 ± 49.12 s \\
    & 4096 & 30/30 & 74.58 ± 15.15 s \\
    & 8192 & 30/30 & 90.06 ± 19.74 s \\
    \bottomrule
    \end{tabular}
    
    \textbf{Tower Stacking with multiple Obstacles}
    \begin{tabular}{lrrr}
    \toprule
    \textbf{Approach} & $N_b$ & \textbf{Coverage} & \textbf{Sol. Time} \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM w/o TrajOpt }} 
    & 512 & 100/100 & 13.87 ± 7.31 ms \\
    & 1024 & 100/100 & \textbf{12.43 ± 4.96 ms} \\
    & 2048 & 100/100 & 15.84 ± 4.55 ms \\
    & 4096 & 100/100 & 34.73 ± 4.13 ms \\
    & 8192 & 100/100 & 84.71 ± 4.81 ms \\
    \midrule
    \multirow{5}{*}{\parbox{1.35cm}{\scshape SPaSM + TrajOpt}} 
    & 512 & 4/5 & \textbf{65.48 ± 30.38 s} \\
    & 1024 & 25/30 & 133.69 ± 61.31 s \\
    & 2048 & 30/30 & 119.91 ± 49.12 s \\
    & 4096 & 30/30 & 74.58 ± 15.15 s \\
    & 8192 & 30/30 & 90.06 ± 19.74 s \\
    \bottomrule
    \end{tabular}

    \caption{10-Tower stacking problem results. As the complexity of the environment increases, SPaSM without trajOpt is unable to find successful solutions. }
    \label{fig:towerstacking}
\end{figure}
